Information Theoretic Representation Distillation

Despite the empirical success of knowledge distillation, current state-of-the-art methods are computationally expensive to train, which makes them difficult to adopt in practice. To address this problem, we introduce two distinct complementary losses inspired by a cheap entropy-like estimator. These losses aim to maximise the correlation and mutual information between the student and teacher representations. Our method incurs significantly less training overheads than other approaches and achieves competitive performance to the state-of-the-art on the knowledge distillation and cross-model transfer tasks. We further demonstrate the effectiveness of our method on a binary distillation task, whereby it leads to a new state-of-the-art for binary quantisation and approaches the performance of a full precision model. Code: www.github.com/roymiles/ITRD

==> sections/limitations.tex <==
% \green{Discussion of Limitations: Considering the limitations of an approach is an important part of good academic scholarship. While many high-quality CVPR papers thoroughly consider and discuss limitations, CVPR 2022 aims to emphasize the importance of an honest treatment of limitations. Authors are thus explicitly encouraged to discuss limitations, ideally by creating a separate "Limitations" (sub-)section in their papers.\footnote{https://cvpr2022.thecvf.com/cmt-submissions-website#papers}} \\

%In this section we discuss some of the limitations of this work and some interesting future directions which are beyond the scope of this paper.
%\begin{enumerate}
%  \paragraph{Limitations} \roy{Reviewer used this against us. Is this even needed?}
% One of the limitations is the slight departure from the underlying theory deriving the matrix-based entropy-like estimators~\cite{SanchezGiraldo2013InformationKernels}. Specifically, the correlation matrix in equation \ref{eqn:cross_corr_c} was not normalised s.t. $A' \circ B'$ would have a trace of $1$. The $\log_2$ is also not used in the mutual information loss. These two modifications were motivated by the empirical performance of the student, however, there is still a close connection between these proposed losses and the entropy-like quantities for which they are maximising.
    
% A lot of the data spatial information is also lost in the final representation. This is the space on which the proposed losses are defined and so may be regarded as a limitation for more structured tasks. We expect that research in this direction to be a natural extension of this work.

==> sections/reproducibility.tex <==
\paragraph{Reproducibility} 
To aid the reproducibility of this work, we implemented ITRD in both the CRD evaluation framework~\cite{Tian2019ContrastiveDistillation} and the \textit{torchdistill}~\cite{Matsubara2020TorchdistillDistillation} KD reproducibility framework, which will both be released. Furthermore, the pseudo-code in algorithm \ref{alg:training_pseudo_code} encapsulates both losses, showing the simplicity of using the proposed losses in current KD settings. We hope that the release of the code, along with the computational simplicity of our approach will encourage further development of this work.
% \paragraph{Limitations and future work.} 
% A large amount of the spatial information is lost by the final representation, which is the space in which the distillation losses are defined. This loss of spatial information may be regarded as a limitation for more structured tasks (\eg, semantic segmentation or object detection), however, we expect that research in this direction would be a natural extension of this work. Another promising direction for this work is in the context of deep mutual learning. Jointly training both the teacher and student models can provide effective collaboration at the cost of increased training time.

% \green{Discussion of Limitations: Considering the limitations of an approach is an important part of good academic scholarship. While many high-quality CVPR papers thoroughly consider and discuss limitations, CVPR 2022 aims to emphasize the importance of an honest treatment of limitations. Authors are thus explicitly encouraged to discuss limitations, ideally by creating a separate "Limitations" (sub-)section in their papers.\footnote{https://cvpr2022.thecvf.com/cmt-submissions-website#papers}} \\

%In this section we discuss some of the limitations of this work and some interesting future directions which are beyond the scope of this paper.
%\begin{enumerate}
%  \paragraph{Limitations} \roy{Reviewer used this against us. Is this even needed?}
% One of the limitations is the slight departure from the underlying theory deriving the matrix-based entropy-like estimators~\cite{SanchezGiraldo2013InformationKernels}. Specifically, the correlation matrix in equation \ref{eqn:cross_corr_c} was not normalised s.t. $A' \circ B'$ would have a trace of $1$. The $\log_2$ is also not used in the mutual information loss. These two modifications were motivated by the empirical performance of the student, however, there is still a close connection between these proposed losses and the entropy-like quantities for which they are maximising.
    
% A lot of the data spatial information is also lost in the final representation. This is the space on which the proposed losses are defined and so may be regarded as a limitation for more structured tasks. We expect that research in this direction to be a natural extension of this work.

==> sections/societal_impact.tex <==
%\paragraph{Potential negative societal impacts} Our work has the potential of reducing the inference cost of current machine learning pipelines. Although this leads to a reduced energy footprint for deep learning models, and also to an improved performance in resource-constrained devices, it also makes it easier to abuse deep learning models for unethical use. However, strictly speaking, this research has applications in many different domains with both positive and negative implications. ITRD is generally applicable in deep learning literature and we specifically focus on tasks which do not have any immediate negative implications.

==> tables/hyper_parameter_search_alpha.tex <==

% RN50 - MN2 - [Not sure if a=0.1 is strictly valid as 1/(1-a) will be +ve]
% a=0.1   [71.39, 71.10] 
% a=1.01  [71.06, 71.39, 70.99] -> [71.15, 0.21]
% a=1.5   [71.32, 71.03, 71.68] -> [71.34, 0.33]
% a=2.0   [71.54, 71.27, 71.46] -> [71.42, 0.39]
% a=3.0   [71.49, 71.17, 71.30] -> [71.32, 0.16]
% a=4.0   [71.29, 71.19, 71.18] -> [71.22, 0.06]
% a=5.0   [70.46, 70.82, 69.96] -> [70.41, 0.43]
% a=10.0  [63.84, 61.54, 63.34] -> [62.91, 1.21]

\resizebox{1.\textwidth}{!}{\begin{tabular}{c|ccccccc}
    \toprule
    $\alpha$ & 1.01 & 1.5 & 2.0 & 3.0 &  4.0 & 5.0 & 10.0 \\
    \midrule
    Mean & 71.15 & 71.34 & 71.42 & 71.32 & 71.22 & 70.41 & 62.91 \\
    Std & 0.21 & 0.33 & 0.39 & 0.16 & 0.06 & 0.43 & 1.21 \\
    \midrule
\end{tabular}}

==> tables/hyper_parameter_search_lambda_1.tex <==
\resizebox{\textwidth}{!}{\begin{tabular}{c|ccccccc}
    \toprule
    $\lambda_1$ & 0.0 & 0.5 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 \\
    \midrule
    Mean & - & - & - & - & - & - & - \\
    Std & - & - & - & - & - & - & - \\
    \midrule
\end{tabular}}

==> tables/hyper_parameter_search_lambda_2.tex <==
\resizebox{\textwidth}{!}{\begin{tabular}{c|ccccccc}
    \toprule
    $\lambda_2$ & 0.0 & 0.5 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 \\
    \midrule
    Mean & - & - & - & - & - & - & - \\
    Std & - & - & - & - & - & - & - \\
    \midrule
\end{tabular}}

==> tables/hyper_parameter_search_sigma.tex <==
\resizebox{\textwidth}{!}{\begin{tabular}{c|cccc}
    \toprule
    $\sigma$ & 1.0 & 0.1 & 0.001 & 0.0001 \\
    \midrule
    Mean & - & - & - & - \\
    Std & - & - & - & - \\
    \midrule
\end{tabular}}

==> tables/imagenet_resnet18.tex <==
\resizebox{\textwidth}{!}{\begin{tabular}{c|cc|cccc|cc|cc|cc}
    \toprule
    & Teacher & Student & AT & KD & 
    % SP & CC & 
    CRD & WCoRD & ReviewKD & FT & SSKD & CRCD & $\mathcal{L}_{corr}$ & $\mathcal{L}_{corr} + \mathcal{L}_{mi}$ \\
    \midrule
    
    Top-1 & 26.69 & 30.25 & 29.30 & 29.34 & 
    % 29.38 & 30.04 & 
    28.62 & 28.44 & 28.39 & 28.57 & 28.38 & \textbf{28.04} & 28.37 & \underline{28.32} \\
    
    Top-5 & 8.58 & 10.93 & 10.00 & 10.12 & 
    % 10.20 & 10.83 & 
    9.51 & 9.45 & 9.49 & 9.71 & 9.33 & \textbf{9.06} & 9.42 & 9.44 \\
    
    \midrule
    % 71.4771
    % 28.52 w/ Lmi log
\end{tabular}}

==> tables/kd_different_architectures.tex <==
\resizebox{0.8\textwidth}{!}{\begin{tabular}{ccccccc}
    \toprule
    \textbf{Teacher} & \textbf{vgg13} & \textbf{ResNet50} & \textbf{ResNet50} & \textbf{resnet32x4} & \textbf{resnet32x4} & \textbf{WRN-40-2} \\
    \textbf{Student} & \textbf{MobileNetV2} & \textbf{MobileNetV2} & \textbf{vgg8} & \textbf{ShuffleNetV1} & \textbf{ShuffleNetV2} & \textbf{ShuffleNetV1} \\
    \midrule
    Teacher & 74.64 & 79.34 & 79.34 & 79.42 & 79.42 & 75.61 \\ 
    Student & 64.60 & 64.60 & 70.36 & 70.50 & 71.82 & 70.50 \\ 
    \midrule
    KD~\cite{Hinton2015DistillingNetwork} & 67.37 & 67.37 & 73.81 & 74.07 & 74.45 & 74.83 \\
    FitNet~\cite{Romero2015FitNets:Nets} & 64.14 (\underperform) & 63.16 (\underperform) & 70.69 (\underperform) & 73.59 (\underperform) & 73.54 (\underperform) & 73.73 (\underperform) \\
    AT~\cite{Zagoruyko2019PayingTransfer} & 59.40 (\underperform) & 58.58 (\underperform) & 71.84 (\underperform) & 71.73 (\underperform) & 72.73 (\underperform) & 73.32 (\underperform) \\
    SP~\cite{Tung2019Similarity-preservingDistillation} & 66.30 (\underperform) & 68.08 (\outperform) & 73.34 (\underperform) & 73.48 (\underperform) & 74.56 (\outperform) & 74.52 (\underperform) \\
    CC~\cite{Peng2019CorrelationDistillation} & 64.86 (\underperform) & 65.43 (\underperform) & 70.25 (\underperform) & 71.14 (\underperform) & 71.29 (\underperform) & 71.38 (\underperform) \\
    VID~\cite{Ahn2019VariationalTransfer} & 65.56 (\underperform) & 67.57 (\outperform) & 70.30 (\underperform) & 73.38 (\underperform) & 73.40 (\underperform) & 73.61 (\underperform) \\
    RKD~\cite{Park2019RelationalDistillation} & 64.52 (\underperform) & 64.43 (\underperform) & 71.50 (\underperform) & 72.28 (\underperform) & 73.21 (\underperform) & 72.21 (\underperform) \\
    PKT~\cite{Passalis2018LearningTransfer} & 67.13 (\underperform) & 66.52 (\underperform) & 73.01 (\underperform) & 74.10 (\outperform) & 74.69 (\outperform) & 73.89 (\underperform) \\
    AB~\cite{Heo2019KnowledgeNeurons} & 66.06 (\underperform) & 67.20 (\underperform) & 70.65 (\underperform) & 73.55 (\underperform) & 74.31 (\underperform) & 73.34 (\underperform) \\
    FT~\cite{Kim2018ParaphrasingTransfer} & 61.78 (\underperform) & 60.99 (\underperform) & 70.29 (\underperform) & 71.75 (\underperform) & 72.50 (\underperform) & 72.03 (\underperform) \\
    NST~\cite{Huang2017LikeTransfer} & 58.16 (\underperform) & 64.96 (\underperform) & 71.28 (\underperform) & 74.12 (\outperform) & 74.68 (\outperform) & 74.89 (\outperform) \\
    CRD~\cite{Tian2019ContrastiveDistillation} & 69.73 (\outperform) & 69.11 (\outperform) & 74.30 (\outperform) & 75.11 (\outperform) & 75.65 (\outperform) & 76.05 (\outperform) \\
    CRD+KD~\cite{Tian2019ContrastiveDistillation} & 69.94 (\outperform) & 69.54 (\outperform) & 74.58 (\outperform) & 75.12 (\outperform) & 76.05 (\outperform) & 76.27 (\outperform) \\
    WCoRD~\cite{Chen2020WassersteinDistillation} & 69.47 (\outperform) & 70.45 (\outperform) & 74.86 (\outperform) & 75.40 (\outperform) & 75.96 (\outperform) & 76.32 (\outperform) \\
    WCoRD+KD~\cite{Chen2020WassersteinDistillation} & 70.02 (\outperform) & 70.12 (\outperform) & 74.68 (\outperform) & 75.77 (\outperform) & 76.48 (\outperform) & 76.68 (\outperform) \\
    % SAD~\cite{Ji2021ShowMatching} & - & n/a & - & - & n/a & n/a \\
    
    % CRCD~\cite{ZhuComplementaryDistillation} & - & - & - & - & - & - \\
    ReviewKD~\cite{ChenDistillingReview} & 70.37 (\outperform) & 69.89 (\outperform) & - & \textbf{77.45} (\outperform) & \textbf{77.78} (\outperform) & \textbf{77.14} (\outperform) \\
    
    % Do not report any of these results, same as CRCD
    % SRRD~\cite{Bulat2021KnowledgeLearning} & - & - & - & - & - & - \\
    
    % \midrule
    % ITKD (1) \scriptsize (memory-bank) & 69.80 (\outperform) & NaN (\outperform) & NaN (\outperform) & NaN (\outperform) & NaN (\outperform) & 77.24 (\outperform) \\
    
    % % (1) uses student memory bank w/ momentum = 0.5
    % ITKD+KD (1) \scriptsize (memory-bank) & NaN & - & - & - & - & 77.06 (\outperform) \\
    
    % ITKD \scriptsize (memory-bank) & 69.95 (\outperform) & - (\outperform) & - (\outperform) & - (\outperform) & - (\outperform) & \textbf{77.40} (\outperform) \\
    
    %%%%%%%%%%%%%%%%% 2. %%%%%%%%%%%%%%%%%
    % \midrule
    % ITKD \scriptsize (before) & 70.19 (\outperform) & 70.88 (\outperform) & 74.82 (\outperform) & 76.41 (\outperform) & \textbf{76.97} (\outperform) & 77.20 (\outperform) \\
    
    % ITRD & \textbf{70.67} (\outperform) & \textbf{71.14} (\outperform) & 75.64 (\outperform) & \underline{76.67} (\outperform) & 76.67 (\outperform) & 77.14 (\outperform) \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    
    \midrule
    $\mathcal{L}_{corr}$ & \underline{70.26} (\outperform) & \textbf{71.58} (\outperform) & \textbf{75.72} (\outperform) & - (\outperform) & 76.99 (\outperform) & 76.80 (\outperform) \\
    
    $\mathcal{L}_{mi}$ & 65.88 (\outperform) & - (\outperform) & - (\outperform) & - (\outperform) & - (\outperform) & - (\outperform) \\
 
    $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ & \textbf{70.76, 70.00} (\outperform) & \underline{71.06, 71.39} (\outperform) & \underline{75.26, 75.71} (\outperform) & - (\outperform) & \underline{77.24, 77.16} (\outperform) & \underline{77.09} (\outperform) \\
       
    % [resnet50-mobilenetv2] 71.25 was using oldschool Lmi
    % Using ^ 3.01
    % $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ \scriptsize RBF & 70.79 (\outperform) & 71.27 (\outperform) & \textbf{75.91} (\outperform) & 76.66 (\outperform) & 77.15 (\outperform) & \textbf{77.32} (\outperform) \\
    
    % Using poly and log
    % teacher train() and ^2.02
    % $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ \scriptsize teacher train & 70.13 (\outperform) & 71.28 (\outperform) & 75.74 (\outperform) & - (\outperform) & - (\outperform) & \textbf{-} (\outperform) \\
    
    \bottomrule
\end{tabular}}

==> tables/kd_large_capacity_gap.tex <==
\begin{tabular}{cccccc}
    \toprule
    Teacher & Student & KD & TAKD & ITRD & ITRD+TAKD \\
    \midrule
    74.41 & 61.37 & 61.41 & 61.82 & 60.96 & \textbf{XXX} \\
    \bottomrule
\end{tabular}
% 60.330 w/ COR + MI
% 60.960 w/ COR only
% 61.050 w/ COR + logit MI

==> tables/kd_self_supervision.tex <==
\resizebox{0.8\textwidth}{!}{\begin{tabular}{ccccccccc}
    \toprule
    \textbf{Teacher} & \textbf{WRN-40-2} & \textbf{WRN-40-2} & \textbf{resnet56} & \textbf{resnet32x4} & \textbf{vgg13} & \textbf{ResNet50} & \textbf{WRN-40-2} & \textbf{resnet32x4} \\
    \textbf{Student} & \textbf{WRN-16-2} & \textbf{WRN-40-1} & \textbf{resnet20} & \textbf{resnet8x4} & \textbf{MobileNetv2} & \textbf{MobileNetV2} & \textbf{ShuffleNetV1} & \textbf{ShuffleNetV2} \\
    \midrule
    Teacher & 76.45 & 76.45 & 73.44 & 79.63 & 74.64 & 79.34 & 76.45 & 79.63 \\ 
    Teacher* & 80.70 & 80.70 & 77.20 & 83.73 & 78.48 & 83.85 & 80.70 & 83.73 \\ 
    Student & 73.56 & 71.95 & 69.62 & 72.95 & 73.51 & 73.51 & 71.74 & 72.96 \\ 
    \midrule
    SSKD & 76.16 & 75.84 & 70.80 & 75.83 & 76.21 & 78.21 & 76.71 & 77.64 \\ 
    HSAKD & 77.20 & 77.00 & 72.58 & 77.26 & 77.45 & 78.79 & 78.51 & 79.93 \\ 
    HSAKD* & \textbf{78.67} & \textbf{78.12} & \textbf{73.73} & 77.69 & \textbf{79.27} & \textbf{79.43} & \textbf{80.11} & \textbf{80.86} \\ 
    \midrule
    CRCD & 76.67 & 75.95 & 73.21 & 76.42 & - & - & - & - \\ 
    \midrule
    % ITRD \scriptsize (old) & 76.27 & - & - & - & - & - & - & - \\ 
    % ITRD* & 77.72 & - & - & \textbf{77.76} & - & - & - & - \\ 
    
    $\mathcal{L}_{corr}$ & - & - & - & - & - & - & - & - \\
    $\mathcal{L}_{mi}$ & - & - & - & - & - & - & - & - \\
    $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ & 76.10 & - & - & - & - & - & - & - \\
    
    \bottomrule
\end{tabular}}


==> tables/kd_shared_architectures.tex <==
\resizebox{1.0\textwidth}{!}{\begin{tabular}{cccccccc}
    \toprule
    \textbf{Teacher} & \textbf{WRN-40-2} & \textbf{WRN-40-2} & \textbf{resnet56} & \textbf{resnet110} & \textbf{resnet110} & \textbf{resnet32x4} & \textbf{vgg13} \\
    \textbf{Student} & \textbf{WRN-16-2} & \textbf{WRN-40-1} & \textbf{resnet20} & \textbf{resnet20} & \textbf{resnet32} & \textbf{resnet8x4} & \textbf{vgg8} \\
    \midrule
    Teacher & 75.61 & 75.61 & 72.32 & 74.31 & 74.31 & 79.42 & 74.64 \\ 
    Student & 73.26 & 71.98 & 69.06 & 69.06 & 71.14 & 72.50 & 70.36 \\ 
    \midrule
    KD~\cite{Hinton2015DistillingNetwork} & 74.92 & 73.54 & 70.66 & 70.67 & 73.08 & 73.33 & 72.98 \\
    FitNet~\cite{Romero2015FitNets:Nets} & 73.58 (\underperform) & 72.24 (\underperform) & 69.21 (\underperform) & 68.99 (\underperform) & 71.06 (\underperform) & 73.50 (\outperform) & 71.02 (\underperform) \\
    AT~\cite{Zagoruyko2019PayingTransfer} & 74.08 (\underperform) & 72.77 (\underperform) & 70.55 (\underperform) & 70.22 (\underperform) & 72.31 (\underperform) & 73.44 (\outperform) & 71.43 (\underperform) \\
    SP~\cite{Tung2019Similarity-preservingDistillation} & 73.83 (\underperform) & 72.43 (\underperform) & 69.67 (\underperform) & 70.04 (\underperform) & 72.69 (\underperform) & 72.94 (\underperform) & 72.68 (\underperform) \\
    CC~\cite{Peng2019CorrelationDistillation} & 73.56 (\underperform) & 72.21 (\underperform) & 69.63 (\underperform) & 69.48 (\underperform) & 71.48 (\underperform) & 72.97 (\underperform) & 70.71 (\underperform) \\
    VID~\cite{Ahn2019VariationalTransfer} & 74.11 (\underperform) & 73.30 (\underperform) & 70.38 (\underperform) & 70.16 (\underperform) & 72.61 (\underperform) & 73.09 (\underperform) & 71.23 (\underperform) \\
    RKD~\cite{Park2019RelationalDistillation} & 73.35 (\underperform) & 72.22 (\underperform) & 69.61 (\underperform) & 69.25 (\underperform) & 71.82 (\underperform) & 71.90 (\underperform) & 71.48 (\underperform) \\
    PKT~\cite{Passalis2018LearningTransfer} & 74.54 (\underperform) & 73.45 (\underperform) & 70.34 (\underperform) & 70.25 (\underperform) & 72.61 (\underperform) & 73.64 (\outperform) & 72.88 (\underperform) \\
    AB~\cite{Heo2019KnowledgeNeurons} & 72.50 (\underperform) & 72.38 (\underperform) & 69.47 (\underperform) & 69.53 (\underperform) & 70.98 (\underperform) & 73.17 (\underperform) & 70.94 (\underperform) \\
    FT~\cite{Kim2018ParaphrasingTransfer} & 73.25 (\underperform) & 71.59 (\underperform) & 69.84 (\underperform) & 70.22 (\underperform) & 72.37 (\underperform) & 72.86 (\underperform) & 70.58 (\underperform) \\
    FSP~\cite{Yim2017ALearning} & 72.91 (\underperform) & n/a & 69.95 (\underperform) & 70.11 (\underperform) & 71.89 (\underperform) & 72.62 (\underperform) & 70.23 (\underperform) \\
    NST~\cite{Huang2017LikeTransfer} & 73.68 (\underperform) & 72.24 (\underperform) & 69.60 (\underperform) & 69.53 (\underperform) & 71.96 (\underperform) & 73.30 (\underperform) & 71.53 (\underperform) \\
    CRD~\cite{Tian2019ContrastiveDistillation} & 75.48 (\outperform) & 74.14 (\outperform) & 71.16 (\outperform) & 71.46 (\outperform) & 73.48 (\outperform) & 75.51 (\outperform) & 73.94 (\outperform) \\
    CRD+KD~\cite{Tian2019ContrastiveDistillation} & 75.64 (\outperform) & 74.38 (\outperform) & 71.63 (\outperform) & 71.56 (\outperform) & 73.75 (\outperform) & 75.46 (\outperform) & 74.29 (\outperform) \\
    WCoRD~\cite{Chen2020WassersteinDistillation} & 75.88 (\outperform) & 74.73 (\outperform) & 71.56 (\outperform) & 71.57 (\outperform) & 73.81 (\outperform) & 75.95 (\outperform) & 74.55 (\outperform) \\
    WCoRD+KD~\cite{Chen2020WassersteinDistillation} & 76.11 (\outperform) & 74.72 (\outperform) & \textbf{71.92} (\outperform) & \underline{71.88} (\outperform) & \underline{74.20} (\outperform) & \underline{76.15} (\outperform) & 74.72 (\outperform) \\
    
    ReviewKD~\cite{ChenDistillingReview} & 76.12 (\outperform) & \underline{75.09} (\outperform) & \underline{71.89} (\outperform) & - (\outperform) & 73.89 (\outperform) & 75.63 (\outperform) & \underline{74.84} (\outperform) \\
    
    % Moved to other table
    % CRCD~\cite{ZhuComplementaryDistillation} & \textbf{76.67} (\outperform) & \textbf{75.95} (\outperform) & \textbf{73.21} (\outperform) & \textbf{72.33} (\outperform) & \textbf{74.96} (\outperform) & \textbf{76.42} (\outperform) & \textbf{74.97} (\outperform) \\
    
    % SAD~\cite{Ji2021ShowMatching} & 75.47 (\outperform) & - & 71.53 (\outperform) & 71.38 (\outperform) & - & - & - \\
    % IE-DML~\cite{HuangRevisitingFramework} & - & - & - & - & 71.64 (\outperform) & - & - \\
    % SRRD~\cite{Bulat2021KnowledgeLearning} & 75.96 (\outperform) & - & - & - & - & - & - \\
    
    % \midrule
    % ITKD & 75.56 (\outperform) & - & 71.37 (\outperform) & \textbf{72.14} (\outperform) & 74.20 (\outperform) & 73.86 (\outperform) & 74.48 (\outperform) \\ 
    % ITKD+KD & 75.01 (\outperform) & - & \textbf{71.93} (\outperform) & 70.81 (\outperform) & 74.02 (\outperform) & 74.03 (\outperform) & 73.74 (\outperform) \\
    
    % \midrule
    % ITKD \scriptsize (double-barlow) & 75.69 (\outperform) & - & 71.56 (\outperform) & 72.05 (\outperform) & 73.90 (\outperform) & 74.36 (\outperform) & 74.14 (\outperform) \\
    
    % \midrule
    % ITKD (1) \scriptsize (memory-bank) & 75.59 (\outperform) & 74.70 (\outperform) & 71.58 (\outperform) & 71.86 (\outperform) & \textbf{74.29} (\outperform) & 74.29 (\outperform) & 74.70 (\outperform) \\
    
    
    %%%%%%%%%%%%%%%%% 1. %%%%%%%%%%%%%%%%%
    % \midrule
    % ITKD \scriptsize (before) & 75.98 (\outperform) & 74.88 (\outperform) & \underline{71.93} (\outperform) & \underline{72.14} (\outperform) & \underline{74.29} (\outperform) & - (\outperform) & 74.77 (\outperform)  \\
    
    % ITRD \scriptsize & \underline{76.18} (\outperform) & \underline{75.39} (\outperform) & \textbf{-} (\outperform) & \textbf{-} (\outperform) & \textbf{-} (\outperform) & 76.28 (\outperform) & 74.97 (\outperform)  \\
    
    % ITRD \scriptsize(+ sampling) \scriptsize & \textbf{-} (\outperform) & \textbf{-} (\outperform) & \textbf{-} (\outperform) & \textbf{-} (\outperform) & \textbf{-} (\outperform) & \textbf{76.63} (\outperform) & \textbf{75.63} (\outperform)  \\
    
    % ITRD \scriptsize(shared embed) \scriptsize & \textbf{-} (\outperform) & \textbf{-} (\outperform) & \textbf{-} (\outperform) & - (\outperform) & 73.84 (\outperform) & - (\outperform) & 75.30 (\outperform)  \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \midrule
    $\mathcal{L}_{corr}$ \scriptsize & \textbf{76.55} (\outperform) & 74.80 (\outperform) & 71.27 (\outperform) & 71.51 (\outperform) & 73.71 (\outperform) & \textbf{76.28} (\outperform) & 74.77 (\outperform)  \\
    
    % $\mathcal{L}_{mi}$ \scriptsize & 74.10 (\underperform) & 72.18 (\underperform) & 68.82 (\underperform) & 68.58 (\underperform) & 70.84 (\underperform) & 73.01 (\underperform) & 70.95 (\underperform)  \\
    
    % All results
    % $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ \scriptsize & \underline{76.14, 76.14, 76.07} (\outperform) & \textbf{75.39, 74.60} (\outperform) & 71.54, 71.41, 71.47 (\outperform) & \textbf{72.31, 72.19, 71.46} (\outperform) & \textbf{74.29, 74.22} (\outperform) & 75.70, 75.94 (\outperform) & \textbf{74.88, 75.06, 74.20} (\outperform)  \\
    
    $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ \scriptsize & \underline{76.12 $\pm$ 0.04} (\outperform) & \textbf{75.39, 74.60} (\outperform) & 71.47 $\pm$ 0.07 (\outperform) & \textbf{ 71.99 $\pm$ 0.46} (\outperform) & \textbf{74.29, 74.22} (\outperform) & 75.70, 75.94 (\outperform) & \textbf{ 74.71 $\pm$ 0.21 } (\outperform)  \\
    
    % $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ \scriptsize RBF \scriptsize & 76.28 (\outperform) & 75.00 (\outperform) & 71.05 (\outperform) & 71.28 (\outperform) & 74.13 (\outperform) & 76.36 (\outperform) & 74.72 (\outperform)  \\
    
    % VGG Lcorr + L2 Lmi [feat_s[-2]]= 74.37
    % $\mathcal{L}_{corr}+\mathcal{L}_{mi}+KD$ \scriptsize & \textbf{-} (\outperform) & \textbf{-} (\outperform) & \textbf{-} (\outperform) & - (\outperform) & - (\outperform) & - (\outperform) & - (\outperform)  \\
    
    % Lambda2 = [1, 10, 100]
    % WRN-40-2 - WRN-16-2 [ | | ]
    % WRN-40-2 - WRN-40-2 [ | | ]
    % resnet56 - resnet20 [ | | ]
    % resnet110 - resnet20 [ | | 71.89, ]
    % resnet110 - resnet32 [74.13, 73.99 | | ]
    % resnet32x4 - resnet8x4 [75.59, 75.50 |]
    % vgg13 - vgg8 [74.65, 74.97 | 74.57, 74.52]
    
    %%%%%%%%%%%%%%%%% 2. %%%%%%%%%%%%%%%%%
    % $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ \scriptsize teacher train \scriptsize & 76.13 (\outperform) & 75.22 (\outperform) & 71.92 (\outperform) & 71.63 (\outperform) & 73.90 (\outperform) & 75.98 (\outperform) & 74.77 (\outperform)  \\
    
    % $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ \scriptsize nesterov \scriptsize & 75.71 (\outperform) & 75.43 (\outperform) & 71.21 (\outperform) & 71.62 (\outperform) & 74.02 (\outperform) & 75.73 (\outperform) & 74.81 (\outperform) \\
    
    % $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ \scriptsize KD $\tau = 0.1$ \scriptsize & 75.74 (\outperform) & 75.93 (\outperform) & 71.46 (\outperform) & 71.40 (\outperform) & 73.67 (\outperform) & 75.55 (\outperform) & 74.57 (\outperform) \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \bottomrule
\end{tabular}}


==> tables/nlp.tex <==
% \begin{tabular}{ccccc}
%     \toprule
%   & &   \multicolumn{2}{c}{\textbf{SQuAD}} & \textbf{SST-2} \\
%     & \textbf{Model} & \textbf{EM} & \textbf{F1} & \textbf{Acc.} \\
%     \midrule
%     & Teacher (BERT) & 81.5 & 88.6 & 92.7 \\ 
%     \midrule
%     \multirow{3}{*}{\begin{sideways} \textbf{T6}\end{sideways}}
%  %   Student & & \\
%     & DistilBERT~\cite{Sanh2019DistilBERTLighter} & 79.1 & 86.9 & 91.3\\
%     & TextBrewer~\cite{Yang2020TextBrewer:Processing} & 80.8 & 88.1 & 92.0 \\
%     & ITRD & \textbf{81.5 } & \textbf{88.5} & 91.9 \\
%     \midrule
%     \multirow{2}{*}{\begin{sideways} \textbf{T3}\end{sideways}}
%   % Student & 61.4 & 72.9 \\
%   & TextBrewer~\cite{Yang2020TextBrewer:Processing} & 76.3 & 84.8 & {89.2} \\
%   &    ITRD & \textbf{77.7} & \textbf{85.8} & \textbf{89.6} \\
%     \bottomrule
% \end{tabular}

% ~\cite{Sanh2019DistilBERTLighter}
% ~\cite{Yang2020TextBrewer:Processing
\small
\begin{tabular}{cccc}
    \toprule
    & \textbf{Model} & \textbf{EM} & \textbf{F1}  \\
    \midrule
    & Teacher (BERT) & 81.5 & 88.6 \\ 
    \midrule
    \multirow{3}{*}{\begin{sideways} \textbf{T6}\end{sideways}}
 %   Student & & \\
    & DistilBERT & 79.1 & 86.9 \\
    & TextBrewer & 80.8 & 88.1 \\
    & ITRD & \textbf{81.5} & \textbf{88.5}\\
    \midrule
    \multirow{2}{*}{\begin{sideways} \textbf{T3}\end{sideways}}
  % Student & 61.4 & 72.9 \\
  & TextBrewer & 76.3 & 84.8 \\
  &    ITRD & \textbf{77.7} & \textbf{85.8} \\
    \bottomrule
\end{tabular}

% \small
% \begin{tabular}{ccccccccc}
%     \toprule
%     & & Teacher (BERT) & DB & TB & ITRD & DB & TB & ITRD  \\
%     \midrule
%     & EM & 81.5 & 88.6 \\ 
%     & F1 & 88.6 & 88.6 \\ 

% %     \midrule
% %     \multirow{3}{*}{\begin{sideways} \textbf{T6}\end{sideways}}
% %  %   Student & & \\
% %     & DistilBERT~\cite{Sanh2019DistilBERTLighter} & 79.1 & 86.9 \\
% %     & TextBrewer~\cite{Yang2020TextBrewer:Processing} & 80.8 & 88.1 \\
% %     & ITRD & \textbf{81.5} & \textbf{88.5}\\
% %     \midrule
% %     \multirow{2}{*}{\begin{sideways} \textbf{T3}\end{sideways}}
% %   % Student & 61.4 & 72.9 \\
% %   & TextBrewer~\cite{Yang2020TextBrewer:Processing} & 76.3 & 84.8 \\
% %   &    ITRD & \textbf{77.7} & \textbf{85.8} \\
%     \bottomrule
% \end{tabular}

==> tables/object_detection_coco.tex <==
\resizebox{0.75\textwidth}{!}{\begin{tabular}{cl|cccccc}
    \toprule
     & Method & mAP & AP50 & AP75 & AP1 & APm & APs \\
    \midrule
    Teacher & Faster R-CNN w/ R50-FPN & 40.22 & 61.02 & 43.81 & 51.98 & 43.53 & 24.16 \\
    Student & Faster R-CNN w/ MV2-FPN & 29.47 & 48.87 & 30.90 & 38.86 & 30.77 & 16.33 \\ 
    % \midrule
    & \;\; w/ KD~\cite{Hinton2015DistillingNetwork} & 30.13 (+0.66) & 50.28 & 31.35 & 39.56 & 31.91 & 16.69 \\
    & \;\; w/ FitNet~\cite{Romero2015FitNets:Nets} & 30.20 (+0.73) & 49.80 & 31.69 & 39.69 & 31.64 & 16.39 \\
    & \;\; w/ FGFI & 31.16 (+1.69) & 50.68 & 32.92 & 42.12 & 32.63 & 16.73 \\
    & \;\; w/ ReviewKD~\cite{ChenDistillingReview} & \textbf{33.71 (+4.24)} & \textbf{53.15} & \textbf{36.13} & \textbf{46.47} & \textbf{35.81} & \textbf{16.77} \\
    & \;\; w/ ITRD & - & - & - & - & - & - \\
    \bottomrule
\end{tabular}}


==> tables/representation_transfer.tex <==
\resizebox{.9\textwidth}{!}{\begin{tabular}{c|c|cccccc|c}
    \toprule
     & Student & KD & AT & FitNet & CRD & CRD+KD & ITRD & Teacher \\

    \midrule
    CIFAR100 $\rightarrow$ STL-10 & 69.7 & 70.9 & 70.7 & 70.3 & 71.6 & 72.2 & \textbf{72.7} & 68.6 \\ 
    CIFAR100 $\rightarrow$ TinyImageNet & 33.7 & 33.9 & 34.2 & 33.5 & 35.6 & 35.5 & \textbf{36.0} & 31.5 \\
    \bottomrule
    
\end{tabular}}

%     \item Lcorr v.s. RKD: -4.6\%
%     \item Lcorr+Lmi v.s. RKD: +6.0\%
%     \item Lcorr v.s. WCoRD: +14.7\%
%     \item Lcorr+Lmi v.s. WCoRD: +23.9\%
%     \item Lcorr v.s. Lcorr+Lmi: +18.9\%
